A converse to Schreier's index-rank formula

In "Subgroups of free profinite groups and large subfields of Q" (Israel J. Math. 39 (1981), no. 1-2, pages 25-45; MR 617288) A. Lubotzky and L. van den Dries raise the question whether a finitely generated, residually finite group is necessarily free if the rank function on its subgroups of finite index satisfies Schreier's well-known index rank relation (see Question 2 on p. 34). I answered this question in 1980 but, so far, I have not published my answer. This note fills the omission; it gives an amended and abridged version of my original proof.

==> Definitions.tex <==
%
\makeatletter
%
%
\def\ab{\mathop{\operator@font ab}\nolimits}
\def\ad{\mathop{\operator@font ad}\nolimits}
\def\Ad{\mathop{\operator@font Ad}\nolimits}
\def\add{\mathop{\operator@font add}\nolimits}
\def\Aff{\mathop{\operator@font Aff}\nolimits}
\def\AG{\mathop{\operator@font AG}\nolimits}
\def\Alt{\mathop{\operator@font Alt}\nolimits}
\def\Ann{\mathop{\operator@font Ann}\nolimits}
\def\Aut {\mathop{\operator@font Aut  }\nolimits}
%
\def\BPL {\mathop{\operator@font BPL  }\nolimits}
%
\def\can {\mathop{\operator@font can  }\nolimits}
\def\card {\mathop{\operator@font card  }\nolimits}
\def\cd{\mathop{\operator@font cd}\nolimits}
\def\ch{\mathop{\operator@font char}\nolimits}
\DeclareMathOperator{\Cohom}{H} 

\def\coker {\mathop{\operator@font coker }\nolimits}
\def\colim {\mathop{\operator@font colim }\nolimits}
\def\core {\mathop{\operator@font core  }\nolimits}

\def\defi {\mathop{\operator@font def }\nolimits}
\def\Der {\mathop{\operator@font Der }\nolimits}
\def\diag {\mathop{\operator@font diag }\nolimits}
\def\dis {\mathop{\operator@font dis }\nolimits}
\def\dom {\mathop{\operator@font dom }\nolimits}
\def\edg {\mathop{\operator@font edg  }\nolimits}

\def\Eu {\mathop{\operator@font E  }\nolimits}
\def\End {\mathop{\operator@font End  }\nolimits}
\def\Ext {\mathop{\operator@font Ext }\nolimits}

\def\face {\mathop{\operator@font face }\nolimits}
\def\Fit {\mathop{\operator@font Fit }\nolimits}
\def\FP {\mathop{\operator@font FP }\nolimits}
\def\Frat {\mathop{\operator@font Frat  }\nolimits}

\def\gp{\mathop{\operator@font gp  }\nolimits}
\def\gcd{\mathop{\operator@font gcd  }\nolimits}
\def\GL{\mathop{\operator@font GL }\nolimits}

\def\Hom {\mathop{\operator@font Hom }\nolimits}
%
\def\id{\mathbbm{1}}
\def\im{\mathop{\operator@font im }\nolimits}
\def\Inn {\mathop{\operator@font Inn  }\nolimits}
\def\Iso{\mathop{\operator@font Iso}\nolimits}
%
\def\lat{\Lambda}
%
\def\md {\mathop{\operator@font md  }\nolimits}
\def\mod{\mathop{\operator@font mod }\nolimits}
\newcommand{\norm}[1]{\| #1\|}

\def\PL {\mathop{\operator@font PL  }\nolimits} 
\DeclareMathOperator{\Perm}{Perm} 

\def\res {\mathop{\operator@font res }\nolimits} 
\def\rk {\mathop{\operator@font rk  }\nolimits} 

\def\sd {\mathop{\operator@font sd  }\nolimits}
\def\sgp {\mathop{\operator@font sgp  }\nolimits}
\def\sign {\mathop{\operator@font sign  }\nolimits}
\def\SL{\mathop{\operator@font SL }\nolimits}
\def\SO{\mathop{\operator@font SOL }\nolimits}
\def\Sol{\mathop{\operator@font Sol }\nolimits}
%
\def\myspan {\mathop{\operator@font span}\nolimits} 
\def\rad {\mathop{\operator@font rad}\nolimits}
\def\stab {\mathop{\operator@font stab  }\nolimits}
\def\supp {\mathop{\operator@font supp  }\nolimits}
\def\SUPP {\mathop{\operator@font SUPP  }\nolimits}
\def\sym {\mathop{\operator@font sym  }\nolimits}
\def\Sym {\mathop{\operator@font Sym  }\nolimits}
\def\Sp{\mathop{\operator@font Sp }\nolimits}

\def\Tor {\mathop{\operator@font Tor  }\nolimits}
\def\TPL {\mathop{\operator@font TPL  }\nolimits}

\def\Val {\mathop{\operator@font Val  }\nolimits}
\def\ver {\mathop{\operator@font ver  }\nolimits} 
%%
%%
\def\B{\mathbb{B}} 
\def\C{\mathbb{C}}
\def\E{\mathbb{E}}
\def\F{\mathbb{F}}
\def\H{\mathbb{H}}
\def\K{\mathbb{K}}
\def\M{\mathbb{M}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\Q{\mathbb{Q}}
\def\R{\mathbb{R}}
\def\s{\mathbb{S}}
\def\U{\mathbb{U}}
\def\Z{\mathbb{Z}}
%
%
%% Calligraphic letters
\let\@@angstroem=\AA    
\let\angstroem=\@@angstroem
\def\AA{\mathcal{A}}
\def\BB{\mathcal{B}}
\def\CC{\mathcal{C}}
\def\DD{\mathcal{D}}
\def\EE{\mathcal{E}}
\def\FF{\mathcal{F}}
\def\GG{\mathcal{G}}
\def\HH{\mathcal{H}}
\def\II{\mathcal{I}}
\def\JJ{\mathcal{J}}
\def\KK{\mathcal{K}}
\def\LL{\mathcal{L}}
\def\MM{\mathcal{M}}
\def\NN{\mathcal{N}}
\def\OO{\mathcal{O}}
\def\PP{\mathcal{P}}
\def\QQ{\mathcal{Q}}
\def\RR{\mathcal{R}}
\def\SS{\mathcal{S}}
\def\TT{\mathcal{T}}
\def\UU{\mathcal{U}}
\def\VV{\mathcal{V}}
\def\WW{\mathcal{W}}
\def\XX{\mathcal{X}}
\def\YY{\mathcal{Y}}
\def\ZZ{\mathcal{Z}}
%
%% Morphisms
%
\newcommand{\mono}{\rightarrowtail}
\newcommand{\incl}{\hookrightarrow}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\iso}{\stackrel{\sim}{\longrightarrow}}
\newcommand{\isoinv}{\stackrel{\sim}{\longleftarrow}}

% useful abbreviations (see LaTeX Companion, page 80)
%
\newcommand{\eg}{e.g., \xspace}
\newcommand{\ie}{i.e., \xspace}
\newcommand{\etc}{etc. \@\xspace}
\newcommand{\cf}{cf. \@\xspace}

%  Various commands
\newcommand{\act}[1]{\,^{#1}}
%
%% Initialisation
\parindent.5cm\parskip0pt
%
\makeatother
\endinput
